Parton Distributions with Theory Uncertainties: General Formalism and First Phenomenological Studies

We formulate a general approach to the inclusion of theoretical uncertainties, specifically those related to the missing higher order uncertainty (MHOU), in the determination of parton distribution functions (PDFs). We demonstrate how, under quite generic assumptions, theory uncertainties can be included as an extra contribution to the covariance matrix when determining PDFs from data. We then review, clarify, and systematize the use of renormalization and factorization scale variations as a means to estimate MHOUs consistently in deep inelastic and hadronic processes. We define a set of prescriptions for constructing a theory covariance matrix using scale variations, which can be used in global fits of data from a wide range of different processes, based on choosing a set of independent scale variations suitably correlated within and across processes. We set up an algebraic framework for the choice and validation of an optimal prescription by comparing the estimate of MHOU encoded in the next-to-leading order (NLO) theory covariance matrix to the observed shifts between NLO and NNLO predictions. We perform a NLO PDF determination which includes the MHOU, assess the impact of the inclusion of MHOUs on the PDF central values and uncertainties, and validate the results by comparison to the known shift between NLO and NNLO PDFs. We finally study the impact of the inclusion of MHOUs in a global PDF determination on LHC cross-sections, and provide guidelines for their use in precision phenomenology. In addition, we also compare the results based on the theory covariance matrix formalism to those obtained by performing PDF determinations based on different scale choices.

==> tables/chi2table_covth_dis_process.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t]
\begin{center}
\renewcommand*{\arraystretch}{1.78}
\footnotesize
\begin{tabular}{|l|c|C{0.8cm}c|C{0.8cm}c|C{0.8cm}c|C{0.8cm}c|}
  \toprule
  \multicolumn{10}{|c|}{ NNPDF3.1 DIS-only fits}    \\
  &    & \multicolumn{4}{c|}{$\chi^2/N_{\rm dat}$}  & \multicolumn{4}{c|}{$\phi$}   \\
 Process & $n_{\rm dat}$ & \multicolumn{2}{c|}{NLO}  & \multicolumn{2}{c|}{NNLO}  & \multicolumn{2}{c|}{NLO}  & \multicolumn{2}{c|}{NNLO}  \\
 &  &  $C$ & $C+S^{(\rm 9pt)}$  &  $C$ & $C+S^{(\rm 9pt)}$ &  $C$ & $C+S^{(\rm 9pt)}$  &  $C$ & $C+S^{(\rm 9pt)}$  \\
\toprule
DIS NC         & 1593 &  1.086  &  1.074     &   1.088     &     1.085   & 0.295   & 0.298    &  0.345  & 0.327      \\
DIS CC        & 552  &  0.978 &  0.889     &   1.105     &    0.935     &  0.494  &  0.472   &  0.641   & 0.523         \\
\midrule
Total       & 2145 &  1.061  &   1.032    &    1.095    &     1.051    & 0.358   & 0.355    &  0.441   &  0.389          \\
\bottomrule
\end{tabular}
\end{center}
\caption{The values of the $\chi^2/N_{\rm dat}$ and of the $\phi$ estimator
  in the NNPDF3.1 DIS-only fits
  with the theory covariance matrix $S^{\rm (9pt)}$, compared to the results based on including only
  the experimental covariance matrix $C$.
  %
  Results are provided both for the NLO and for the NNLO fits.
  %
  \label{table:chi2table_covth_dis}
}
  \end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> tables/chi2table_covth_global_nlo_process.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t]
\begin{center}
\renewcommand*{\arraystretch}{1.78}
\footnotesize
\begin{tabular}{|l|c|c|ccc|cc|c|}
  \toprule
  &    & \multicolumn{7}{c|}{$\chi^2/n_{\rm dat}$ in the NNPDF3.1 global fits}   \\
 Process & $n_{\rm dat}$ & \multicolumn{6}{c|}{NLO}  & NNLO  \\
 &  & $C$ & $C+S^{(\rm 9pt)}$   &  $C+S^{(\rm 7pt)}$  &  $C+S^{(\rm 3pt)}$ & $C+S^{(\rm 9pt)}_{\rm fit}$ &
  $C+S^{(\rm 9pt)}_{\rm sampl}$   &  $C$ \\
\toprule
DIS NC    & 1593 & 1.088  & 1.079   & 1.086 & 1.095 & 1.081 & 1.227 & 1.084 \\
DIS CC    & 552  & 1.012  & 0.928   & 0.933 & 0.960 & 0.929 & 1.036 & 1.079 \\
\midrule  
DY        & 484  & 1.486  & 1.447   & 1.485 & 1.483 & 1.461 & 1.434 & 1.231 \\
JETS      & 164  & 0.907  & 0.839   & 0.858 & 0.901 & 0.848 & 0.911 & 0.950 \\
TOP       & 26   & 1.260  & 1.012   & 1.016 & 1.077 & 1.001 & 1.264 & 1.068 \\
\midrule
Total     & 2819 & 1.139  & 1.109   & 1.129 & 1.139 & 1.113 & 1.217 & 1.105 \\
\bottomrule
\end{tabular}
\end{center}
\caption{The values of the $\chi^2/N_{\rm dat}$ and of the $\phi$ estimator
  in the NNPDF3.1 global fits
  with the theory covariance matrix $S$, compared to the results based on including only
  the experimental covariance matrix $C$. Results are shown
for  the 9-, 7-, and 3- point prescriptions.
  %
  For the 9-point prescription we also show  results obtained
  including the theory covariance matrix
only in the $\chi^2$ definition Eq.~(\ref{eq:chi2_v3}) but not
in the data generation Eq.~(\ref{eq:dgen}) and conversely.
  Values corresponding to the
  NNLO fit with  experimental covariance matrix $C$ only are also shown.
  \label{table:chi2table_covth_global_nlo}
}
  \end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> tables/chi2table_dis_nnlo.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{center}
\renewcommand*{\arraystretch}{1.7}
\footnotesize
\begin{tabular}{|l|c|ccccccccc|}
  \toprule
Dataset  &  $N_{\rm dat}$ & \multicolumn{9}{c|}{$\chi^2/N_{\rm dat}$ NNPDF3.1 DIS-only NNLO}  \\
  &  & (1,1) & (2,2)  &  $(\half,\half)$  &  (2,1) & (1,2) &  $(1,\half)$ & $(\half,1)$ & $(2,\half)$ & $(\half,2)$  \\
\toprule
NMC  &  134           & 1.244     & 1.229   &  1.231 &  1.244  &   1.263  & 1.231  & 1.266  & 1.291  & 1.289      \\
SLAC  &  12           & 0.794    & 0.850   &  0.894  & 0.794   &  0.829  & 0.801  & 0.740  & 0.551  & 0.720       \\
BCDMS  &  530         & 1.046     & 1.059   &  1.050  & 1.046   &  1.049  & 1.059  & 1.056  & 1.120  & 1.049       \\
CHORUS  &  430        & 1.093     & 1.112   &  1.075  & 1.093   &  1.096  & 1.080  & 1.128  & 1.177  & 1.164       \\
NuTeV  &   41         & 0.892    & 0.781   &  0.597  & 0.892   &  0.673  & 0.754  & 0.634  & 0.808  & 0.712       \\
HERA incl  &  967     & 1.103     & 1.113   &  1.107  & 1.103   &  1.106  & 1.111  & 1.100  & 1.148  & 1.103       \\
HERA $F_2^c$  &  31   &  1.055    & 1.075   &  1.026  & 1.055   &  1.081  & 1.113  & 1.306  & 2.301  & 1.566        \\  
\midrule
Total  &  2145       & 1.089      & 1.098   &  1.082  & 1.089   &  1.090  & 1.091  & 1.097  & 1.163 & 1.111     \\
\bottomrule
\end{tabular}
\end{center}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> tables/chi2table_phi_global_process.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t]
\begin{center}
\renewcommand*{\arraystretch}{1.78}
\footnotesize
\begin{tabular}{|l|c|ccc|cc|c|}
  \toprule
  & \multicolumn{7}{c|}{$\phi$ in the NNPDF3.1 global fits}   \\
 Process & \multicolumn{6}{c|}{NLO}  & NNLO  \\
 & $C$ & $C+S^{(\rm 9pt)}$   &  $C+S^{(\rm 7pt)}$  &  $C+S^{(\rm 3pt)}$ & $C+S^{(\rm 9pt)}_{\rm fit}$ &
  $C+S^{(\rm 9pt)}_{\rm sampl}$   &  $C$ \\
\toprule
DIS NC    & 0.266  & 0.268   & 0.262 & 0.261 & 0.261 & 1.137 & 0.305 \\
DIS CC    & 0.389  & 0.376   & 0.367 & 0.391 & 0.369 & 0.502 & 0.471 \\
\midrule  
DY        & 0.361  & 0.343   & 0.340 & 0.358 & 0.349 & 0.603 & 0.380 \\
JETS      & 0.295  & 0.312   & 0.279 & 0.291 & 0.298 & 0.461 & 0.392 \\
TOP       & 0.375  & 0.352   & 0.318 & 0.331 & 0.319 & 0.612 & 0.363 \\
\midrule
Total     & 0.314  & 0.315   & 0.304 & 0.313 & 0.309 & 0.932 & 0.362 \\
\bottomrule
\end{tabular}
\end{center}
\caption{Same as Table~\ref{table:chi2table_covth_global_nlo}, but 
  for the values of the $\phi$ estimator.
  \label{table:phitable_covth_global_nlo}
}
  \end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> tables/dataset_efficiencies_9pt.tex <==
\begin{tabular}{l|l|l|c}
Prescription & Process & Data set & Efficiency, $\varepsilon$  \\
\hline
    9-pt & DIS NC & NMCPD & 0.84 \\
	& & NMC & 0.87 \\
	& & SLACP & 0.38 \\
	& & SLACD & 6.7 $\times 10^{-3}$ \\
	& & BCDMSP & 0.80 \\
	& & BCDMSD & 0.78 \\
	& & HERAF2CHARM & 0.97 \\
	& & HERACOMBNCEM & 0.70 \\
	& & HERACOMBNCEP460 & 0.83 \\
	& & HERACOMBNCEP575 & 0.83 \\
	& & HERACOMBNCEP820 & 0.95 \\
	& & HERACOMBNCEP920 & 0.73 \\
	\hline
	& DIS CC & NTVNUDMN & 0.92 \\
	& & NTVNBDMN & 0.94 \\
	& & CHORUSNU & 0.86 \\
	& & CHORUSNB & 0.78 \\
	& & HERACOMBCCEM & 0.89 \\
	& & HERACOMBCCEP & 0.86 \\
	\hline
	& DY & ATLASWZRAP36PB & 0.99 \\
	& & ATLASZHIGHMASS49FB & 1.4 $\times 10^{-5}$ \\
	& & ATLASLOMASSDY11EXT & 1.1 $\times 10^{-6}$ \\
	& & ATLASWZRAP11 & 0.99 \\
	& & ATLASZPT8TEVMDIST & 0.99 \\
	& & ATLASZPT8TEVYDIST & 0.99 \\
	& & CMSWEASY840PB & 0.99 \\
	& & CMSWMASY47FB & 0.99 \\
	& & CMSDY2D11 & 0.98 \\
	& & CMSWMU8TEV & 0.99 \\
	& & CMSZDIFF12 & 0.99 \\
	& & LHCBZ940PB & 0.99 \\
	& & LHCBZEE2FB & 0.98 \\
	& & LHCBWZMU7TEV & 0.99 \\
	& & LHCBWZMU8TEV & 0.99 \\
	& & CDFZRAP & 0.91 \\
	& & D0ZRAP & 0.73 \\
	& & D0WEASY & 1.0 \\
	& & D0WMASY & 1.0 \\
	\hline
	& Jets & ATLAS1JET11 & 1.0 \\
	& & CMSJETS11 & 0.99 \\
	\hline
	& Top & ATLASTTBARTOT & -1.0 \\
	& & ATLASTOPDIFF8TEVTRAPNORM & 0.99 \\
	& & CMSTTBARTOT & -0.94 \\
	& & CMSTOPDIFF8TEVTTRAPNORM & 0.92 \\
\end{tabular}


==> tables/pairwise_efficiencies_9pt.tex <==
\begin{tabular}{l|l|c}
Prescription & Processes & Efficiency, $\varepsilon$  \\
\hline
    9-pt & DIS NC + DIS CC & 0.52 \\
	& DIS NC + DY & 0.48 \\
	& DIS NC + Jets & 0.51 \\
	& DIS NC + Top & 0.48 \\
	& DIS CC + DY & 0.64 \\
	& DIS CC + Jets & 0.75 \\
	& DIS CC + Top & 0.71 \\
	& DY + Jets & 0.89 \\
	& DY + Top & 0.85 \\
	& Jets + Top & 0.99 \\
\end{tabular}

